Making data center computations fast, but not so furious

We propose an aggressive computational sprinting variant for data center environments. While most of previous work on computational sprinting focuses on maximizing the sprinting process while ensuring non-faulty conditions, we take advantage of the existing replication in data centers to push the system beyond its safety limits. In this paper we outline this vision, we survey existing techniques for achieving it, and we present some design ideas for future work in this area.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

# SAMPLES = \
# 	sample-manuscript.tex \
# 	sample-acmsmall.tex \
# 	sample-acmlarge.tex \
# 	sample-acmtog.tex \
# 	sample-sigconf.tex \
# 	sample-siggraph.tex \
# 	sample-sigplan.tex \
# 	sample-sigchi.tex \
# 	sample-sigchi-a.tex
SAMPLES = 	main.tex

PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE)

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> conclusion.tex <==
\section{Conclusion/directions}
\daniel{single paragraph summarizing the whole thing}

\daniel{conclusions/directions: sistematic approach to overcloking, leverage
	replication in distributed systems to employ data center sprinting.}
\daniel{stragger mitigation, some times is faster and cheaper sprint then spin off 	replicas or buy new hardware (oversubscription)}
\daniel{block chain}

-----------
CONCLUSION:
combine sprinting with fault tolerance have many advantages:
- stateless computation can benefit from it (examples ...)
- map reduce jobs 
- can reduce straglers by coordinating sprinters (make one of the replicas a
safeguard or a clean up...)
- spike mitigation help while new replicas starts up...
- energy plan.

take aways: how operating systems can be modified to take advantage of
overcloking in trade of more faults... ( Android governor to make the stable
4.0Ghz chip to confiogure to 4.7GhZ but force it to work at 4.0 until is
necessary or triggered to operate in 4.7) 


